Cross-domain Imitation from Observations

Imitation learning seeks to circumvent the difficulty in designing proper reward functions for training agents by utilizing expert behavior. With environments modeled as Markov Decision Processes (MDP), most of the existing imitation algorithms are contingent on the availability of expert demonstrations in the same MDP as the one in which a new imitation policy is to be learned. In this paper, we study the problem of how to imitate tasks when there exist discrepancies between the expert and agent MDP. These discrepancies across domains could include differing dynamics, viewpoint, or morphology; we present a novel framework to learn correspondences across such domains. Importantly, in contrast to prior works, we use unpaired and unaligned trajectories containing only states in the expert domain, to learn this correspondence. We utilize a cycle-consistency constraint on both the state space and a domain agnostic latent space to do this. In addition, we enforce consistency on the temporal position of states via a normalized position estimator function, to align the trajectories across the two domains. Once this correspondence is found, we can directly transfer the demonstrations on one domain to the other and use it for imitation. Experiments across a wide variety of challenging domains demonstrate the efficacy of our approach.

==> 3_method.bak.tex <==
We aim to learn a correspondence across two domains: an expert domain, on which we have demonstrations and the agent domain, on which we wish to learn the policy. Consider an infinite horizon Markov Decision Process (MDP) $\mathcal{M}=\left(\mathcal{S},\mathcal{A},\mathcal{P},r,\gamma,\mathcal{P}_0\right)$, where $\mathcal{S}$ is the state space, $\mathcal{A}$ is the action space, $\mathcal{P}$ is the dynamics or transition function, $r$ is the reward function, $\gamma \in (0,1)$ is the discount factor and $\mathcal{P}_0$ is the initial state distribution. Following \cite{kim2020domain}, we define a domain as an MDP without the reward, i.e., $\left(\mathcal{S},\mathcal{A},\mathcal{P},\gamma,\mathcal{P}_0\right)$ - thus, the domain typifies the agent morphology and the dynamics, but not the desired behavior. Augmenting a domain with a reward describes an MDP aimed at solving the task corresponding to the specified reward. We define an MDP in some domain $x$ for task $\mathcal{T}$ as $\mathcal{M}_x^\mathcal{T}=\left(\mathcal{S}_x,\mathcal{A}_x,\mathcal{P}_x,r_x^\mathcal{T},\gamma_x,\mathcal{P}_{0x}\right)$. A trajectory corresponding to task $\mathcal{T}$ in domain $x$ is a sequence of states $\eta_{\mathcal{M}_x^\mathcal{T}}=\{s_x^0,s_x^1,\dots,s_x^{H_{\eta}}\}$, where $H$ denotes the length of the trajectory; $\mathcal{D}_{\mathcal{M}_x^\mathcal{T}}=\{\eta^i_{\mathcal{M}_x^\mathcal{T}}\}_{i=1}^N$ denotes a set of such trajectories.
